Robust Handwriting Recognition with Limited and Noisy Data

Despite the advent of deep learning in computer vision, the general handwriting recognition problem is far from solved. Most existing approaches focus on handwriting datasets that have clearly written text and carefully segmented labels. In this paper, we instead focus on learning handwritten characters from maintenance logs, a constrained setting where data is very limited and noisy. We break the problem into two consecutive stages of word segmentation and word recognition respectively and utilize data augmentation techniques to train both stages. Extensive comparisons with popular baselines for scene-text detection and word recognition show that our system achieves a lower error rate and is more suited to handle noisy and difficult documents

==> tables/data.tex <==
% % \iffalse
% \begin{table}[t!]
% \ra{1.2}
% \centering 
% %\begin{tabular}{llllllll}
% \begin{tabular}{l*3{c}}
% \toprule 
% Type         &       Train     & Val     &   Test  \\ 
% \hline
% Segmentation &    $40,159$  &  $641$     &  $721$      \\ 
% Classification &    $660,000$    &  $3,400$  &  - \\ 
% \bottomrule 
% \end{tabular}
% \caption{Statistics of Segmentation and Classification datasets. For Segmentation, each sample is a form (as an image) that contains multiple words. For Classification, each sample is an image that contains a single word. All data are annotated from our BHP dataset.}
% \label{tbl:data}
% \end{table}




% \fi
% % \newcolumntype{K}[1]{>{\centering\arraybackslash}p{#1}}

% % \begin{table}[t!]
% % %\vspace{-5mm}
% % \caption{Dataset Statistics}
% % \centering
% % \label{tbl:data}
% % \fontsize{8.5}{10}\selectfont
% % \vspace{-2mm}
% % \begin{tabular}{|c||*{3}{K{1.2cm}}|}
% % \hline
% % Model         &       Train(\%)     & Val(\%)     &   Test(\%)  \\ 
% % Ours (Yelp 1)   &  \textbf{60.1}  &  \textbf{60.1} &   59.4   \\
% % Ours (Yelp 2)   &  62.3 &  60.5  &  \textbf{57.7}  \\ \hline
% % \end{tabular}
% % % \vspace{-5mm}
% % \end{table}




==> tables/pipeline.tex <==
\begin{table}[t!]
\ra{1.2}
\centering 
\begin{tabular}{@{}lllll@{}}
\toprule
Class & Real Only & Synthetic Only & Mixed Data & \\
\midrule
Word   & 0.890  & 0.086 & 0.894 \\
\midrule
Signature   & 0.782  & 0.000 & 0.753 \\
\midrule
Stamp   & 0.899  & 0.000 & 0.842 \\
\midrule
Date   & 0.829  & 0.000 & 0.753 \\
\midrule
Noise   & 0.174  & 0.000 & 0.198 \\
\bottomrule
\end{tabular}
\caption{Full pipeline results attained by choosing the best models from Segmentation and Recognition models. }
\label{tbl:multimodels}
\end{table}

==> tables/sota.tex <==
\begin{table*}[t]
\fontsize{9}{11}\selectfont
\setlength\tabcolsep{1.0pt}
\centering
\caption{More language modeling results using AWD-LSTM on Penn Treebank. Using domain knowledge to infer sparse structures helps to reduce the embedding parameters by $100\times$. Ppl: perplexity, \# Emb: \# (non-zero) embedding parameters.}
\begin{tabular}{l | c c c c c | c | c}
\Xhline{3\arrayrulewidth}
\multirow{1}{}{Method} & \multirow{1}{}{$|A|$} & \multirow{1}{}{Init $A$} & \multirow{1}{}{Sparse $\mathbf{T}$} & \multirow{1}{}{\textsc{Relu}($\mathbf{T}$)} & \multirow{1}{}{Domain} & \multicolumn{1}{c|}{Ppl} & \multicolumn{1}{c}{\# Emb (M)}\\
% ({\color{gg}{\boldmath$\downarrow$}})
\Xhline{0.5\arrayrulewidth}
%\multirow{5}{*}{\makecell{{\color{blue}{Vocab}}\\ {\color{blue}{selection}}}}
AWD-LSTM~\citep{DBLP:journals/corr/abs-1708-02182} & $10,000$ & All  & \textcolor{rr}\xmark & \textcolor{rr}\xmark & \textcolor{rr}\xmark & $59.0$ & $4.00$\\
\Xhline{0.5\arrayrulewidth}
%\multirow{6}{*}{\makecell{{\color{rr}{Anchor \&}}\\ {\color{rr}{Transform}}}}
% All 10000:		59 ppl		10000x400	4 million
% Frequency 100:	70 ppl		100x400 and 9900x1000 with ~10000 non zero
% Frequency 1000:	77 ppl		1000x400 and 9000x1000 with ~50000 non zero
% Random 1000:	72 ppl		1000x400 and 10000x1000 with ~40000 non zero
\multirow{3}{*}{{\color{rr}{}}}
& $1,000$ & Dynamic   & \textcolor{gg}\cmark & \textcolor{gg}\cmark & \textcolor{rr}\xmark & $72.0$ & $0.44$\\
& $1,000$ & Frequency   & \textcolor{gg}\cmark & \textcolor{gg}\cmark & \textcolor{rr}\xmark & $77.0$ & $0.45$\\
& $100$ & Frequency & \textcolor{gg}\cmark & \textcolor{gg}\cmark & \textcolor{gg}\cmark & $\mathbf{70.0}$ & $\mathbf{0.05}$\\
\Xhline{3\arrayrulewidth}
\end{tabular}
\vspace{-4mm}
\label{lm_supp}
\end{table*}
